Translate-and-Revise: Boosting Large Language Models for Constrained Translation

Imposing constraints on machine translation systems presents a challenging issue because these systems are not trained to make use of constraints in generating adequate, fluent translations. In this paper, we leverage the capabilities of large language models (LLMs) for constrained translation, given that LLMs can easily adapt to this task by taking translation instructions and constraints as prompts. However, LLMs cannot always guarantee the adequacy of translation, and, in some cases, ignore the given constraints. This is in part because LLMs might be overly confident in their predictions, overriding the influence of the constraints. To overcome this overiding behaviour, we propose to add a revision process that encourages LLMs to correct the outputs by prompting them about the constraints that have not yet been met. We evaluate our approach on four constrained translation tasks, encompassing both lexical and structural constraints in multiple constraint domains. Experiments show 15\% improvement in constraint-based translation accuracy over standard LLMs and the approach also significantly outperforms neural machine translation (NMT) state-of-the-art methods.

==> figs/different_llm.tex <==
%这个图用到了\usepackage{pgfplots} 和 \usetikzlibrary{patterns}这两个包
\makeatletter
\newcommand\resetstackedplotsnew{
    \makeatletter
    \pgfplots@stacked@isfirstplottrue
    \makeatother
    \addplot [forget plot,draw=none] coordinates{(Qwen, 0) (ChatGPT, 0) (GPT-3, 0) (GPT-4, 0)};
}
% \makeatother
\begin{minipage}{0.5\textwidth}
\flushleft
\begin{tikzpicture} [scale=0.40]
\tikzstyle{every node}=[font=\large]
\begin{axis} [
% title={en-ru},
% ybar,
ybar stacked,
ylabel=\LARGE CCR\%,
ymin=60,
ymax=100,
xtick = data,
xticklabel style={rotate=-14, anchor=center, xshift=0em, yshift=-1.5em},
bar width=.58cm,
enlarge x limits=0.17,
% nodes near coords,
symbolic x coords={Qwen, ChatGPT, GPT-3, GPT-4},
legend style={ legend columns=-1,
    column sep = 0.6em,
    /tikz/column 2/.style={column sep=2em,},
    at={(0.9,1.1)},
    anchor=south,
    draw=none}, 
]
\addplot [bar shift=-.35cm,
    draw = black,
    semithick,
    pattern = north east lines,
    pattern color = black
] coordinates {(ChatGPT,85.9) (GPT-3,72.7) (GPT-4,85.9) (Qwen,75.5)};

\resetstackedplotsnew

\addplot [bar shift=.25cm,
    draw = blue,
    semithick,
    pattern = north east lines,
    pattern color = blue
] coordinates {(ChatGPT,95.8) (GPT-3,92.2) (GPT-4,96.6) (Qwen,88.0)};

\addplot [bar shift=.25cm,
    draw = red,
    semithick,
    pattern = north east lines,
    pattern color = red
] coordinates {(ChatGPT,1.7) (GPT-3,5.6) (GPT-4,1.2) (Qwen,5.0)};

\legend {\LARGE w/o TAR , \LARGE TAR w/o revision};
\end{axis} 

\node (lang)[anchor=north,font=\scriptsize] at ([xshift=10em,yshift=-10em]it.north){En-Ru};

\end{tikzpicture}
\end{minipage}%
\begin{minipage}{0.30\textwidth}
\begin{tikzpicture}[scale=0.40]
\tikzstyle{every node}=[font=\large]
\begin{axis} [
% title={en-zh},
% ybar,
ybar stacked,
ylabel=\LARGE CCR\%,
ymin=60,
ymax=100,
xtick = data,
xticklabel style={rotate=-14, anchor=center, xshift=0em, yshift=-1.5em},
bar width=.58cm,
enlarge x limits=0.17,
% nodes near coords,
symbolic x coords={Qwen, ChatGPT, GPT-3, GPT-4},
legend style={ legend columns=-1,
    column sep = 0.6em,
    at={(0.4,1.08)},
    anchor=south,
    draw=none}, 
]
\addplot [bar shift=-.35cm,
    draw = black,
    semithick,
    pattern = north east lines,
    pattern color = black
] coordinates {(ChatGPT,87.2) (GPT-3,81.6) (GPT-4,85.2) (Qwen,83.5)};

\resetstackedplotsnew

\addplot [bar shift=.25cm,
    draw = blue,
    semithick,
    pattern = north east lines,
    pattern color = blue
] coordinates {(ChatGPT,92.6) (GPT-3,91.6) (GPT-4,94.5) (Qwen,92.6)};

\addplot [bar shift=.25cm,
    draw = red,
    semithick,
    pattern = north east lines,
    pattern color = red
] coordinates {(ChatGPT,2.9) (GPT-3,4.8) (GPT-4,2.0) (Qwen,1.4)};

\legend {, , \LARGE TAR};
\end{axis}
\node (lang)[anchor=north,font=\scriptsize] at ([xshift=10em,yshift=-10em]it.north){En-Zh};
\end{tikzpicture}
\end{minipage}%

==> tables/lexically_constrained_trans_main_res.tex <==
\begin{table}[t!]
\small
    % \centering

\resizebox{1.0\linewidth}{!}{
    \begin{tabular}{l|ll|ll}
        \toprule
        \textbf{\large Method} & \textbf{\large BLEU} & \textbf{\large CCR\%} & \textbf{\large BLEU} & \textbf{\large CCR\%} \\
        \midrule
        \textit{Dataset} & \multicolumn{2}{c|}{\textit{IATE}} & \multicolumn{2}{c}{\textit{Wiktionary}} \\
        \midrule
        Transformer        & 25.8 & 76.3 & 26.0 & 76.9 \\
        Const. Dec.  & 25.3 & 82.0 & 25.8 & \textbf{99.5} \\
        Source. Fact.     & 26.0 & 94.5 & 26.3 & 93.4  \\
        % TADA        & 27.1 & 98.0 & 26.7 & 96.8  \\
        RTT & 27.2 & \textbf{99.6} & 27.8 & 98.3  \\
        LLM Trans.     & \textbf{32.0} & 85.4 & \textit{32.0} & 88.7  \\
        \midrule
        LLM Const. Trans. & \textbf{32.0} & 96.2 & \textbf{32.1} & 97.2  \\
        \rowcolor{black!20}
        \quad +Revision & \textbf{32.0\textsubscript{(+0.0)}} & \textit{98.9\textsubscript{(+2.7)}}  & \textit{32.0\textsubscript{(-0.1)}}  & \textit{98.9\textsubscript{(+1.7)}}  \\
        % NMT Trans.     & \textit{35.3} & 85.4 & \textit{35.3} & 90.3  \\
        % \rowcolor{black!20}
        % \quad +Revision& \textbf{35.5\textsubscript{(+0.2)}} & 98.0\textsubscript{(+12.6)}  & \textbf{35.5\textsubscript{(+0.2)}}  & 97.9\textsubscript{(+7.6)}  \\
        \bottomrule
    \end{tabular} 
   }

    \caption{Results of the general lexically constrained translation task. The \textbf{highest} scores among the various systems are highlighted in bold, while the \textit{second-best} scores are emphasized in italics for clarity.}

    \label{tab:dinu_res}
    
\vspace{-1.1em}

\end{table}

==> tables/terminology_trans_main_res.tex <==
% 因为这四个表都用到了灰色高亮,所以复制到别的工程的话要把头文件的\usepackage{xcolor}改成\usepackage[table]{xcolor}不然加载不出来！！！切记！！！> <
\begin{table}[t!]
\small
    \centering

\resizebox{1.0\linewidth}{!}{
    \begin{tabular}{l|ll|ll}
        \toprule
        \textbf{\large Method} & \textbf{\large BLEU} & \textbf{\large CCR\%} & \textbf{\large BLEU} & \textbf{\large CCR\%} \\
        \midrule
        \textit{Direction} & \multicolumn{2}{c|}{\textit{English-Chinese}} & \multicolumn{2}{c}{\textit{English-Russian}} \\
        \midrule
        HW-TSC        & \textbf{40.7} & 88.6 & - & - \\
        TermMind-sys2  & \textit{40.5} & 85.6 & - & - \\
        ProMT.soft     & - & - & \textbf{31.1} & 90.9  \\
        TildeMT        & - & - & 28.2 & 86.3  \\
        Lingua Custodia & 29.6 & 82.8 & 28.8 & 85.4  \\
        LLM Trans.     & 36.3 & 87.2 & 29.7 & 85.9  \\
        \midrule
        LLM Const. Trans. & 36.4 & \textit{92.6} & 30.1 & \textit{95.8}  \\
        \rowcolor{black!20}
        \quad +Revision & 35.9\textsubscript{(-0.5)} & \textbf{95.9\textsubscript{(+3.3)}}  & \textit{30.3\textsubscript{(+0.2)}}  & \textbf{97.5\textsubscript{(+1.7)}}  \\
        % NMT Trans.     & 34.5 & 85.6 & \textit{33.6} & 85.3  \\
        % \rowcolor{black!20}
        % \quad +Revision& 35.2\textsubscript{(+0.7)} & \textit{95.6\textsubscript{(+10)}}  & \textbf{34.0\textsubscript{(+0.4)}}  & \textit{96.6\textsubscript{(+11.3)}}  \\
        \bottomrule
    \end{tabular} 
   }

    \caption{Results of the terminology translation task for both English-Chinese and English-Russian. }

    \label{tab:term_res}
    
\vspace{-1.1em}

\end{table}
